Stochastic Quasi-Gradient Methods: Variance Reduction via Jacobian Sketching

We develop a new family of variance reduced stochastic gradient descent methods for minimizing the average of a very large number of smooth functions. Our method --JacSketch-- is motivated by novel developments in randomized numerical linear algebra, and operates by maintaining a stochastic estimate of a Jacobian matrix composed of the gradients of individual functions. In each iteration, JacSketch efficiently updates the Jacobian matrix by first obtaining a random linear measurement of the true Jacobian through (cheap) sketching, and then projecting the previous estimate onto the solution space of a linear matrix equation whose solutions are consistent with the measurement. The Jacobian estimate is then used to compute a variance-reduced unbiased estimator of the gradient. Our strategy is analogous to the way quasi-Newton methods maintain an estimate of the Hessian, and hence our method can be seen as a stochastic quasi-gradient method. We prove that for smooth and strongly convex functions, JacSketch converges linearly with a meaningful rate dictated by a single convergence theorem which applies to general sketches. We also provide a refined convergence theorem which applies to a smaller class of sketches. This enables us to obtain sharper complexity results for variants of JacSketch with importance sampling. By specializing our general approach to specific sketching strategies, JacSketch reduces to the stochastic average gradient (SAGA) method, and several of its existing and many new minibatch, reduced memory, and importance sampling variants. Our rate for SAGA with importance sampling is the current best-known rate for this method, resolving a conjecture by Schmidt et al (2015). The rates we obtain for minibatch SAGA are also superior to existing rates.

==> sec-trash.tex <==
\clearpage

\section{Sampling With Replacement:  $\tau$--array collection}

\peter{Need to introduce this again, just here, and using the new narrative and language.}

Let $\cG$ be the $\tau$--array collection.


The smoothness $\LGconst$ is defined completely analogously to~\eqref{eq:LGsmoothwithoutrep} except now the average is taken over arrays  thus
\begin{equation}\label{eq:LGsmoothwithrep}
\LGconst \eqdef \max_{i=1,\ldots,n} \frac{1}{n^{\tau-1}} \sum_{C \, :\, C \in \cG, \, i \in C} L_C, \end{equation}
since there are now $n^{\tau -1}$ elements in the set $\{C \, :\, C \in \cG, \, i \in C\}$, where we use $i \in C$ to denote that there exists $\mJ$ such that $C_j =i.$



When $\mW = \mD_L$, from~\eqref{eq:rhoarraycollectW} and~\eqref{eq:stepsizeuniform} if the stepsize satisfies
\begin{equation}\label{eq:stepsizearray}
\alpha \leq  \frac{1}{4}\min\left\{ \frac{1}{ \LGconst }, \, \frac{\tau }{   \frac{n-\tau}{n} L_{\max}+ \bar{L}  +\frac{\mu}{4} n   }\right\},
\end{equation}
then the resulting iteration complexity~\eqref{eq:itercompluni} is given by
\begin{equation}\label{eq:aos8j38j8j}
\frac{4}{\mu}\max \left\{ \LGconst, \,
 \frac{n-\tau}{ n\tau} L_{\max}  +\frac{1}{\tau}\bar{L} + \frac{\mu}{4}\frac{n}{\tau} \right\},
\end{equation}
%
where we used 
\[ \frac{1}{\tau}\sum_{j\neq \max} L_j \leq \frac{n}{\tau} \, \bar{L},\]
to simplfiy the presentation.


When $\mW=\mI$, inserting~\eqref{eq:rhoarraycollectI} into~\eqref{eq:stepsizeuniform}, if the stepsize satisfies
\begin{equation}\label{eq:stepsizearrayI}
\alpha  \leq    \frac{1}{4}\min\left\{ \frac{1}{\LGconst }, \, \frac{1 }{ \frac{n-\tau+1}{n\tau}L_{\max}    +\frac{\mu}{4} \frac{n}{\tau}   }\right\},
\end{equation}
then Theorem~\ref{theo:convgen} guarantees a resulting iteration complexity of
\begin{eqnarray}
\boxed{\frac{4}{\mu}\max \left\{ \LGconst, \,
\frac{n-\tau+1}{n\tau}L_{\max}    +\frac{\mu}{4} \frac{n}{\tau}\right \} .} \label{eq:itercomplarrayI}
\end{eqnarray}
Note that since $\frac{1}{n\tau} L_{\max} \leq \frac{1}{\tau} \bar{L}$ we have that~\eqref{eq:itercomplarrayI} is a better iteration complexity than~\eqref{eq:aos8j38j8j}. 

\section{More obsolete stuff}


\begin{itemize}
\item$\mS = \mI_S$,  where $S$ is a sampling, and  $\mI_S \in \R^{n\times |S|}$ is a column submatrix of the $n\times n$ identity matrix $\mI$ associated with columns indexed by the set $S$. That is, $\Prb{\mS = \mI_C} = p_{C}$ for all $C\subseteq [n]$. Assume that $\mW=\mI$. Note that then
% \[\Proj_{\mI_S} \overset{\eqref{eq:PSdef}}{=} \mI_S \left( \mI_S^\top \mW \mI_S\right)^{-1} \mI_S^\top \mW = \mI_S \mI_S^\top.\]
%In particular, $\Proj_{\mI_C}$ is independent of $\mW$.

 \begin{equation} \label{eq:n8g7v00hvf} \Proj_{\mS}  = \Proj_{\mI_S} \overset{\eqref{eq:PSdef}}{=} \mI_S \left( \mI_S^\top \mI_S\right)^{-1} \mI_S^\top = \mI_S \mI_S^\top.\end{equation}
 
\item $\mS = e_S$.
That is, $\Prb{\mS = e_C} = p_{C}$ for all $C\subseteq [n]$. Assume that $\mW=\mI$. Note that then
 \begin{equation} \label{eq:ubif9879hd8} \Proj_{\mS}  = \Proj_{e_S} \overset{\eqref{eq:PSdef}}{=} e_S \left( e_S^\top e_S\right)^{-1} e_S^\top  \overset{\eqref{eq:e_C}}{=} \frac{1}{|S|} e_S e_S^\top.\end{equation}
\end{itemize}



If $\mS =e_S$, then this follows from \eqref{eq:e_C} since  $e_S^\top \ones = |S|$. 

\begin{lemma}\label{lem:circsimp} For any constant $C \in \R$ the matrix $M = \ones \ones^\top + C I$ has only two distinct eigenvalues given by $\lambda_1 = C$ and $\lambda_2 =C+n$
\end{lemma}
\begin{proof} The matrix $M$ can be re-written as
 $\mM = C(\mI-\frac{\ones \ones^\top}{n}) + (n+C)\frac{\ones \ones^\top}{n},$ thus $\mM$ is a sum of two scaled mutually orthogonal projection matrices. Consequently the eigenspaces of $M$ are given by
$E_1 = \Range\ones$ and $E_2 = \Range\ones^\perp$ with associated eigenvalues $\lambda_1 =C$  and $\lambda_2 = C+n$, respectively.
\end{proof}

